Towards Adversarially Robust Deep Metric Learning

Deep Metric Learning (DML) has shown remarkable successes in many domains by taking advantage of powerful deep neural networks. Deep neural networks are prone to adversarial attacks and could be easily fooled by adversarial examples. The current progress on this robustness issue is mainly about deep classification models but pays little attention to DML models. Existing works fail to thoroughly inspect the robustness of DML and neglect an important DML scenario, the clustering-based inference. In this work, we first point out the robustness issue of DML models in clustering-based inference scenarios. We find that, for the clustering-based inference, existing defenses designed DML are unable to be reused and the adaptions of defenses designed for deep classification models cannot achieve satisfactory robustness performance. To alleviate the hazard of adversarial examples, we propose a new defense, the Ensemble Adversarial Training (EAT), which exploits ensemble learning and adversarial training. EAT promotes the diversity of the ensemble, encouraging each model in the ensemble to have different robustness features, and employs a self-transferring mechanism to make full use of the robustness statistics of the whole ensemble in the update of every single model. We evaluate the EAT method on three widely-used datasets with two popular model architectures. The results show that the proposed EAT method greatly outperforms the adaptions of defenses designed for deep classification models.

==> experiments.tex <==
\section{Experiments}

In this work, we consider the adversarial example attack in the DML tasks under the white-box setting (which means the attacker knows the structure and the parameters of the deep learning model). In this section, we first evaluate our EAT defense on three widely used datasets (CUB200, CARS196, and In-Shop) with two popular models (MobileNetV2 and BN-Inception). We then study effect of hyperparameters on CUB200 and CARS196. 

\subsection{Dataset}
We evaluate our methods on CUB200\cite{WelinderEtal2010}, CARS196\cite{KrauseStarkDengFei-Fei_3DRR2013} and In-Shop\cite{liuLQWTcvpr16DeepFashion}. CUB200 is an image dataset with photos of 200 bird species. For CUB200, we select its first 100 classes which contain 2944 images as our training set and other 3089 images of the other classes as our test set. CARS196 is an image dataset with 196 classes of cars. For the CARS196, we choose the 8054 images of its first 98 classes as our training set and the other 8131 images are used for testing. For the In-Shop, we use its first 3997 classes which contain 25882 images for training and the other 28760 images are used for testing. The test set of the In-Shop consists of two parts: the query part and the gallery part. The query part contains 14218 images of 3986 classes and the gallery part has 12612 images of 3985 classes. In this work, we only select the query part as the test data to analyze the robustness like the test part of CUB200 and CARS196.

\subsection{Model}
In this work, we select the MobileNetV2\cite{DBLP:journals/corr/abs-1801-04381} and the BN-Inception\cite{DBLP:journals/corr/IoffeS15} as the deep learning model to train and test. In every experiment, we all use the corresponding pre-trained model on the ImageNet\cite{imagenet_cvpr09} as the initial model before the training phase. At the beginning of the training step, we re-initialize the parameters of the final full connection layer for each model.

\subsection{Evaluation Metric}
In the evaluation phase, we exploit three metrics (Recall, F1-Score, and NMI) to evaluate the performance of the deep learning model in DML tasks.

The form of the recall value can be written as:
\begin{equation}
    Recall = \frac{TP}{TP+FN}
\end{equation}
where $TP$ is the true-positive counts and the $FN$ is the false-negative counts. In the DML tasks, we often use $Recall@k$ for evaluating the performance when considering top-$k$ predictions.

The form of the F1-Score is:
\begin{equation}
    \text{F1-Score} = \frac{2TP}{2TP+FN+FP}
\end{equation}
where $FP$ is the false-positive counts. The F1-Score is the combination of recall and precision.

The NMI value is the Normalized Mutual Information. That value can measure the quality of the clustering and is widely used in metric learning tasks. The form of the NMI can be written as:
\begin{equation}
    NMI(\Omega, C) = \frac{2\mathbb{I}(\Omega, C)}{H(\Omega)+H(C)}
\end{equation}
where $\Omega$ is the class label, $C$ is the cluster label, $\mathbb{I}(\cdot, \cdot)$ is the mutual information function and $H(\cdot)$ is the entropy function.

\subsection{Implementation Detail}

During the training step, we exploit the AdamW\cite{DBLP:journals/corr/abs-1711-05101} optimizer which has the same update process of the Adam\cite{kingma2014adam} yet decays the weights separately to perform the backpropagation.
Our models are trained for 200 epochs with the initial learning rate $10^{-4}$ on three datasets. We apply the learning rate scheduler to adjust the learning rate during the training
phase. During the training phase, we set the PGD attack with $\varepsilon = 16/255$ and the iteration number is set as 10. In the test phase, we set $\varepsilon = 8/255$ and the iteration number is also set as 10.

For all the input images, we resize them to the size of 256x256 and make the central crop on them for obtaining final images with the size of 224x224.
We also apply the normalization on these images with the means vector $(0.485, 0.456, 0.406)$ and the std vector $(0.229, 0.224, 0.225)$. As for the implementation, our code is based on the work of Roth et al. \cite{roth2020revisiting} and the defense work of Pang et al. \cite{pangMixupInferenceBetter2020}.

In this work, we select Proxy Anchor Loss (PAL) \cite{kimProxyAnchorLoss2020} as the metric learning loss because that loss has got SOTA performance in metric learning tasks. The PAL has the same form as the triplet loss and it can be written as:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{pal} =& \frac{1}{|P^+|} \sum_{p\in P^+} [{g(LSE_{x\in X_p^+}(-\alpha(s(x,p)-m))}] \\
    &+ \frac{1}{|P|}\sum_{p\in P}[g(LSE_{x\in X_p^-}(\alpha(s(x,p)+m))] 
\end{aligned}
\end{equation}

where $m > 0$ is the margin, $\alpha$ is the scaling factor, $P$ is the set of all proxies, $P^+$ denotes all the positive proxies, $g(x)=\log(1+e^x)$ is the softplus function and $LSE$ is the Log-Sum-Exp operation. For each proxy $p$, $X_p^+$ is the set of all positive samples of $p$ and $X^-_p = X - X_p^+$. $s(x,y) = \text{cossim}(\mathcal{F}(x),\mathcal{F}(y))$ and $\text{cossim}(x,y) = \frac{x\cdot y}{||x||||y||}$ is the cosine similarity function.

% Based on the PAL, our problem can be rewritten with a concise style as:
% \begin{equation}
%     \begin{aligned}
%     \min \mathbb{E}_{X\sim D} \Big[\max_{X_{adv}\sim S(X,\varepsilon)} \mathcal{L}_{pal}(X;\mathcal{F}(\cdot;\theta))\Big]
%     \end{aligned}
% \end{equation}


\subsection{Result Analysis}

\textbf{The adversarial robustness comparison of all defenses.} As is shown in Table \ref{tab:mobi-cub200-cars196} to Table \ref{tab:bn-in-shop}, four kinds of defenses all obtain great performance under the clean mode (i.e. without any attacks). These defenses all cause a little drop of all metrics after the training phase. The AT method presents minimum performance drop under the clean mode and the Mix-Up method shows maximum drop without any attacks. As for the adversarial robustness of these defenses, the Mix-Up method and the IAT method fail under the PGD attack with 10 iterations with a huge drop of all the metrics. Our proposed EAT defense presents the SOTA performance under the PGD attack. Especially on the recall metric, our EAT defense outperforms the AT method.

\begin{table*}[]
\begin{center}
\begin{adjustbox}{width=((\columnwidth)*2),center}
\begin{tabular}{cc|cccccc|cccccc}
\hline
Method                                 &                       & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        \\ \hline
                                       & \multicolumn{1}{l|}{} & \multicolumn{6}{c|}{CUB200}                                                                               & \multicolumn{6}{c}{CARS196}                                                                              \\ \hline
\multirow{2}{*}{\textbf{PAL}}          & Clean                 & 59.97          & 22.73          & 53.27          & 64.15          & 74.47          & 84.03          & 51.02          & 16.16          & 51.40          & 63.52          & 74.59          & 84.73          \\ \cline{2-14} 
                                       & PGD-10                & 30.95          & 1.73          & 7.16          & 10.84          & 16.17          & 23.89          & 27.10          & 1.97          & 5.52          & 8.89          & 14.22          & 23.09          \\ \hline
\multirow{2}{*}{\textbf{PAL + AT}}     & Clean                 & 59.52          & 21.15          & 53.24          & 63.52          & 73.71          & 82.68          & 48.29          & 14.18          & 39.97          & 52.60          & 64.87          & 76.28          \\ \cline{2-14} 
                                       & PGD-10                & 35.54          & 3.58          & 17.98          & 23.89          & 32.53          & 43.12          & 31.72          & 4.18          & 14.15          & 20.28          & 28.68          & 38.80          \\ \hline
\multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean                 & 56.70          & 18.58          & 51.66          & 62.34          & 72.92          & 82.29          & 47.89          & 12.89          & 45.00          & 58.15          & 69.58          & 80.33          \\ \cline{2-14} 
                                       & PGD-10                & 31.32          & 2.01          & 8.77          & 12.88          & 18.86          & 26.85          & 28.11          & 2.20          & 7.26          & 11.85          & 18.47          & 28.83          \\ \hline
\multirow{2}{*}{\textbf{PAL + IAT}}    & Clean                 & 57.67          & 19.68          & 51.36          & 62.21          & 72.66          & 82.16          & 52.90          & 16.39          & 56.02          & 67.95          & 77.55          & 85.66          \\ \cline{2-14} 
                                       & PGD-10                & 32.27          & 2.39          & 12.32          & 17.78          & 24.55          & 33.49          & 31.35          & 3.62          & 14.41          & 21.60          & 30.49          & 40.80          \\ \hline
\multirow{2}{*}{\textbf{PAL + EAT}}    & Clean                 & 56.91          & 19.28          & 52.78          & 62.34          & 71.31          & 80.48          & 51.23          & 14.95          & 54.68          & 65.18          & 74.69          & 83.09          \\ \cline{2-14} 
                                       & PGD-10                & \textbf{38.02} & \textbf{4.84} & \textbf{24.02} & \textbf{30.43} & \textbf{37.56} & \textbf{47.49} & \textbf{36.08} & \textbf{5.77} & \textbf{22.80} & \textbf{31.52} & \textbf{42.46} & \textbf{54.21} \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\caption{The comparison of four defenses on the CUB200 and the CARS196 with the MobileNetV2 under the white-box adversarial example attack. Noted that the PAL + AT is the same as previous defense proposed by \citeauthor{baiAdversarialMetricAttack2020} and \citeauthor{panumExploringAdversarialRobustness2021}}
\label{tab:mobi-cub200-cars196}
\end{table*}

\begin{table*}[]
\begin{center}
\begin{adjustbox}{width=((\columnwidth)*2),center}
\begin{tabular}{cc|cccccc|cccccc}
\hline
Method                                 &                       & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        \\ \hline
                                       & \multicolumn{1}{l|}{} & \multicolumn{6}{c|}{CUB200}                                                                               & \multicolumn{6}{c}{CARS196}                                                                              \\ \hline
\multirow{2}{*}{\textbf{PAL}}          & Clean                 & 58.17          & 20.15          & 55.01          & 66.41          & 75.68          & 84.26          & 54.18          & 18.08          & 60.42          & 71.46          & 80.58          & 87.59          \\ \cline{2-14} 
                                       & PGD-10                & 31.88          & 2.35          & 11.53          & 16.60          & 23.83          & 33.26          & 27.19          & 2.29          & 9.26          & 15.05          & 22.72          & 33.84          \\ \hline
\multirow{2}{*}{\textbf{PAL + AT}}     & Clean                 & 57.20          & 20.23          & 53.73          & 64.08          & 74.17          & 82.85          & 56.64          & 19.92          & 67.82          & 78.01          & 86.02          & 91.01          \\ \cline{2-14} 
                                       & PGD-10                & 36.17          & 4.25          & 21.75          & 28.03          & 36.61          & 46.76          & 34.99          & 5.46          & 28.59          & 37.97          & 48.06          & 59.59          \\ \hline
\multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean                 & 58.67          & 20.68          & 55.14          & 66.09          & 75.48          & 84.23          & 53.63          & 17.90          & 60.93          & 71.17          & 80.16          & 88.20          \\ \cline{2-14} 
                                       & PGD-10                & 31.14          & 2.10          & 11.80          & 16.63          & 23.60          & 33.36          & 27.41          & 2.29          & 10.36          & 16.25          & 24.07          & 35.57          \\ \hline
\multirow{2}{*}{\textbf{PAL + IAT}}    & Clean                 & 57.19          & 19.64          & 53.57          & 64.15          & 74.30          & 83.21          & 56.07          & 18.74          & 67.65          & 77.28          & 85.29          & 91.45          \\ \cline{2-14} 
                                       & PGD-10                & 36.42          & 4.49          & 21.10          & 28.16          & 35.75          & 45.19          & 34.53          & 5.23          & 27.95          & 37.65          & 48.18          & 58.93          \\ \hline
\multirow{2}{*}{\textbf{PAL + EAT}}    & Clean                 & 56.65          & 19.67          & 55.93          & 65.76          & 74.14          & 82.75          & 55.41          & 19.20          & 69.56          & 77.77          & 84.39          & 89.96          \\ \cline{2-14} 
                                       & PGD-10                & \textbf{38.42} & \textbf{4.89} & \textbf{25.50} & \textbf{32.67} & \textbf{40.32} & \textbf{50.25} & \textbf{37.10} & \textbf{6.14} & \textbf{34.86} & \textbf{43.64} & \textbf{53.24} & \textbf{63.52} \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\caption{The comparison of four defenses on the CUB200 and the CARS196 with the BN-Inception under the white-box adversarial example attack.}
\label{tab:bn-cub200-cars196}
\end{table*}

% \begin{table}[ht]
% \begin{center}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{cccccccc}
% \hline
% Method                                 &        & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        \\ \hline
% \multirow{2}{*}{\textbf{PAL}}          & Clean  & 0.5997          & 0.2273          & 0.5327          & 0.6415          & 0.7447          & 0.8403          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3095          & 0.0173          & 0.0716          & 0.1084          & 0.1617          & 0.2389          \\ \hline
% \multirow{2}{*}{\textbf{PAL + AT}}     & Clean  & 0.5952          & 0.2115          & 0.5324          & 0.6352          & 0.7371          & 0.8268          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3554          & 0.0358          & 0.1798          & 0.2389          & 0.3253          & 0.4312          \\ \hline
% \multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean  & 0.5670          & 0.1858          & 0.5166          & 0.6234          & 0.7292          & 0.8229          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3132          & 0.0201          & 0.0877          & 0.1288          & 0.1886          & 0.2685          \\ \hline
% \multirow{2}{*}{\textbf{PAL + IAT}}    & Clean  & 0.5767          & 0.1968          & 0.5136          & 0.6221          & 0.7266          & 0.8216          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3227          & 0.0239          & 0.1232          & 0.1778          & 0.2455          & 0.3349          \\ \hline
% \multirow{2}{*}{\textbf{PAL + EAT}}    & Clean  & 0.5691          & 0.1928          & 0.5278          & 0.6234          & 0.7131          & 0.8048          \\ \cline{2-8} 
%                                       & PGD-10 & \textbf{0.3802} & \textbf{0.0484} & \textbf{0.2402} & \textbf{0.3043} & \textbf{0.3756} & \textbf{0.4749} \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{center}
% \caption{The comparison of four defenses on the CUB200 with the MobileNetV2 under the white-box adversarial example attack.}
% \label{tab:mob-cub200}
% \end{table}


% \begin{table}[ht]
% \begin{center}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{cccccccc}
% \hline
% Method                                 &        & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        \\ \hline
% \multirow{2}{*}{\textbf{PAL}}          & Clean  & 0.5817          & 0.2015          & 0.5501          & 0.6641          & 0.7568          & 0.8426          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3188          & 0.0235          & 0.1153          & 0.1660          & 0.2383          & 0.3326          \\ \hline
% \multirow{2}{*}{\textbf{PAL + AT}}     & Clean  & 0.5720          & 0.2023          & 0.5373          & 0.6408          & 0.7417          & 0.8285          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3617          & 0.0425          & 0.2175          & 0.2803          & 0.3661          & 0.4676          \\ \hline
% \multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean  & 0.5867          & 0.2068          & 0.5514          & 0.6609          & 0.7548          & 0.8423          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3114          & 0.0210          & 0.1180          & 0.1663          & 0.2360          & 0.3336          \\ \hline
% \multirow{2}{*}{\textbf{PAL + IAT}}    & Clean  & 0.5719          & 0.1964          & 0.5357          & 0.6415          & 0.7430          & 0.8321          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3642          & 0.0449          & 0.2110          & 0.2816          & 0.3575          & 0.4519          \\ \hline
% \multirow{2}{*}{\textbf{PAL + EAT}}    & Clean  & 0.5665          & 0.1967          & 0.5593          & 0.6576          & 0.7414          & 0.8275          \\ \cline{2-8} 
%                                       & PGD-10 & \textbf{0.3842} & \textbf{0.0489} & \textbf{0.2550} & \textbf{0.3267} & \textbf{0.4032} & \textbf{0.5025} \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{center}
% \caption{The comparison of four defenses on the CUB200 with the BN-Inception under the white-box adversarial example attack.}
% \label{tab:bn-cub200}
% \end{table}

% \begin{table}[h]
% \begin{center}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{cccccccc}
% \hline
% Method                                 &        & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        \\ \hline
% \multirow{2}{*}{\textbf{PAL}}          & Clean  & 0.5102          & 0.1616          & 0.5140          & 0.6352          & 0.7459          & 0.8473          \\ \cline{2-8} 
%                                       & PGD-10 & 0.2710          & 0.0197          & 0.0552          & 0.0889          & 0.1422          & 0.2309          \\ \hline
% \multirow{2}{*}{\textbf{PAL + AT}}     & Clean  & 0.4829          & 0.1418          & 0.3997          & 0.5260          & 0.6487          & 0.7628          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3172          & 0.0418          & 0.1415          & 0.2028          & 0.2868          & 0.3880          \\ \hline
% \multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean  & 0.4789          & 0.1289          & 0.4500          & 0.5815          & 0.6958          & 0.8033          \\ \cline{2-8} 
%                                       & PGD-10 & 0.2811          & 0.0220          & 0.0726          & 0.1185          & 0.1847          & 0.2883          \\ \hline
% \multirow{2}{*}{\textbf{PAL + IAT}}    & Clean  & 0.5290          & 0.1639          & 0.5602          & 0.6795          & 0.7755          & 0.8566          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3135          & 0.0362          & 0.1441          & 0.2160          & 0.3049          & 0.4080          \\ \hline
% \multirow{2}{*}{\textbf{PAL + EAT}}    & Clean  & 0.5123          & 0.1495          & 0.5468          & 0.6518          & 0.7469          & 0.8309          \\ \cline{2-8} 
%                                       & PGD-10 & \textbf{0.3608} & \textbf{0.0577} & \textbf{0.2280} & \textbf{0.3152} & \textbf{0.4246} & \textbf{0.5421} \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{center}
% \caption{The comparison of four defenses on the CARS196 with the MobileNetV2 under the white-box adversarial example attack.}
% \label{tab:mob-cars196}
% \end{table}

% \begin{table}[h]
% \begin{center}
% \begin{adjustbox}{width=\columnwidth,center}
% \begin{tabular}{cccccccc}
% \hline
% Method                                 &        & NMI             & F1-Score        & Recall@1        & Recall@2        & Recall@4        & Recall@8        \\ \hline
% \multirow{2}{*}{\textbf{PAL}}          & Clean  & 0.5418          & 0.1808          & 0.6042          & 0.7146          & 0.8058          & 0.8759          \\ \cline{2-8} 
%                                       & PGD-10 & 0.2719          & 0.0229          & 0.0926          & 0.1505          & 0.2272          & 0.3384          \\ \hline
% \multirow{2}{*}{\textbf{PAL + AT}}     & Clean  & 0.5664          & 0.1992          & 0.6782          & 0.7801          & 0.8602          & 0.9101          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3499          & 0.0546          & 0.2859          & 0.3797          & 0.4806          & 0.5959          \\ \hline
% \multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean  & 0.5363          & 0.1790          & 0.6093          & 0.7117          & 0.8016          & 0.8820          \\ \cline{2-8} 
%                                       & PGD-10 & 0.2741          & 0.0229          & 0.1036          & 0.1625          & 0.2407          & 0.3557          \\ \hline
% \multirow{2}{*}{\textbf{PAL + IAT}}    & Clean  & 0.5607          & 0.1874          & 0.6765          & 0.7728          & 0.8529          & 0.9145          \\ \cline{2-8} 
%                                       & PGD-10 & 0.3453          & 0.0523          & 0.2795          & 0.3765          & 0.4818          & 0.5893          \\ \hline
% \multirow{2}{*}{\textbf{PAL + EAT}}    & Clean  & 0.5541          & 0.1920          & 0.6956          & 0.7777          & 0.8439          & 0.8996          \\ \cline{2-8} 
%                                       & PGD-10 & \textbf{0.3710} & \textbf{0.0614} & \textbf{0.3486} & \textbf{0.4364} & \textbf{0.5324} & \textbf{0.6352} \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{center}
% \caption{The comparison of four defenses on the CARS196 with the BN-Inception under the white-box adversarial example attack.}
% \label{tab:bn-cars196}
% \end{table}


\begin{table}[]
\begin{center}
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ccccccccc}
\hline
Method                                 &        & NMI             & F1-Score        & Recall@1        & Recall@10       & Recall@20       & Recall@30        & \multicolumn{1}{l}{Recall@40} \\ \hline
\multirow{2}{*}{\textbf{PAL}}          & Clean  & 86.88          & 14.95          & 60.97          & 82.69          & 86.70          & 88.81          & 90.12                        \\ \cline{2-9} 
                                       & PGD-10 & 82.47          & 3.36          & 16.25          & 32.86          & 39.05          & 42.87          & 45.45                        \\ \hline
\multirow{2}{*}{\textbf{PAL + AT}}     & Clean  & 86.71          & 14.19          & 57.29          & 80.41          & 84.79          & 87.30          & 88.70                        \\ \cline{2-9} 
                                       & PGD-10 & 84.68          & 8.51          & 38.06          & 62.46          & 69.20          & 73.07          & 75.47                        \\ \hline
\multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean  & 86.88          & 14.85          & 60.77          & 82.75          & 86.68          & 88.71          & 89.96                        \\ \cline{2-9} 
                                       & PGD-10 & 82.46          & 3.43          & 16.66          & 33.44          & 39.53          & 43.51          & 46.38                        \\ \hline
\multirow{2}{*}{\textbf{PAL + IAT}}    & Clean  & 86.76          & 14.37          & 57.98          & 80.86          & 85.54          & 87.72          & 89.08                        \\ \cline{2-9} 
                                       & PGD-10 & 84.78          & 8.80          & 38.27          & 63.03          & 69.72          & 73.55          & 76.15                        \\ \hline
\multirow{2}{*}{\textbf{PAL + EAT}}    & Clean  & 86.82          & 14.40          & 58.69          & 79.58          & 84.34          & 86.57          & 87.97                        \\ \cline{2-9} 
                                       & PGD-10 & \textbf{85.30} & \textbf{10.03} & \textbf{43.16} & \textbf{66.16} & \textbf{72.64} & \textbf{75.88} & \textbf{78.23}               \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\caption{The comparison of four defenses on the In-Shop with the MobileNetV2 under the white-box adversarial example attack.}
\label{tab:mob-in-shop}
\end{table}

\begin{table}[]
\begin{center}
    \begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{ccccccccc}
\hline
Method                                 &        & NMI             & F1-Score        & Recall@1        & Recall@10       & Recall@20       & Recall@30        & \multicolumn{1}{l}{Recall@40} \\ \hline
\multirow{2}{*}{\textbf{PAL}}          & Clean  & 87.45          & 16.41          & 67.22          & 87.59          & 91.03          & 92.71          & 93.73                        \\ \cline{2-9} 
                                       & PGD-10 & 82.60          & 3.88          & 20.57          & 40.74          & 47.91          & 52.26          & 55.27                        \\ \hline
\multirow{2}{*}{\textbf{PAL + AT}}     & Clean  & 87.14          & 15.35          & 62.45          & 84.55          & 88.70          & 90.65          & 91.93                        \\ \cline{2-9} 
                                       & PGD-10 & 85.43          & 10.26          & 44.79          & 71.78          & 78.13          & 81.40          & 83.60                        \\ \hline
\multirow{2}{*}{\textbf{PAL + Mix-Up}} & Clean  & 87.58          & 16.78          & 68.01          & 87.75          & 91.17          & 92.88          & 93.93                        \\ \cline{2-9} 
                                       & PGD-10 & 82.49          & 3.82          & 20.76          & 41.60          & 48.53          & 52.65          & 55.84                        \\ \hline
\multirow{2}{*}{\textbf{PAL + IAT}}    & Clean  & 87.19          & 15.54          & 62.86          & 84.55          & 88.46          & 90.55          & 91.98                        \\ \cline{2-9} 
                                       & PGD-10 & 85.50          & 10.45          & 44.91          & 72.20          & 78.39          & 81.66          & 83.77                        \\ \hline
\multirow{2}{*}{\textbf{PAL + EAT}}    & Clean  & 87.35          & 15.75          & 66.17          & 84.47          & 88.39          & 90.27          & 91.64                        \\ \cline{2-9} 
                                       & PGD-10 & \textbf{86.18} & \textbf{12.10} & \textbf{52.74} & \textbf{75.69} & \textbf{81.17} & \textbf{83.81} & \textbf{85.74}               \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\caption{The comparison of four defenses on the In-Shop with the BN-Inception under the white-box adversarial example attack.}
\label{tab:bn-in-shop}
\end{table}

\textbf{The adversarial robustness under different iteration numbers of the attack.} As is shown in Figure \ref{fig:iter-recall@1-f1-mobi-cub200}, our proposed EAT defense presents the SOTA adversarial robustness than other defenses under the PGD attack with different iteration numbers.  
Under the PGD attack, the Mix-Up method is close to the No Defense. That means the effect of the Mix-Up method is small and it is not suitable for applying that kind of method in the DML tasks. The F1-Score and the Recall@1 decrease when we increasing the iteration number of the PGD attack but there are some fluctuations due to the randomness. 

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/iter-recall@1-mobi-cub200.png}
% \end{center}
%   \caption{Recall@1 for different iteration numbers of the PGD attack with the different defenses on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:iter-recall@1-mobi-cub200}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/iter-f1-mobi-cub200.png}
% \end{center}
%   \caption{F1-Score for different iteration numbers of the PGD attack with the different defenses on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:iter-f1-mobi-cub200}
% \end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/iter-recall@1-f1-mobi-cub200.png}
\end{center}
  \caption{Recall@1 and F1-Score for different iteration numbers of the PGD attack with the different defenses on the CUB200 dataset (Training with the MobileNetV2)}
\label{fig:iter-recall@1-f1-mobi-cub200}
\end{figure}

\textbf{The robustness under different attack budgets $\varepsilon$ settings.} We evaluate our EAT defense in comparison with the other defenses under different $\varepsilon$ settings (8/255, 12/255, 16/255, 20/255, 24/255, 28/255, and 32/255). As is shown in Figure \ref{fig:eps-recall@1-f1-mobi-cub200}, the EAT defense still outperforms other defenses. The F1-Score and the Recall@1 decrease when increasing the $\varepsilon$ of the PGD attack. There are also some fluctuations due to the randomness of the iteration step. 

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/recall@1-eps-cub200.png}
% \end{center}
%   \caption{Recall@1 for different $\varepsilon$ settings of the PGD attack with the different defenses on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:recall@1-eps-cub200}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/f1-eps-cub200.png}
% \end{center}
%   \caption{F1-Score for different $\varepsilon$ settings of the PGD attack with the different defenses on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:f1-eps-cub200}
% \end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/eps-recall1-f1-mobi-cub200.png}
\end{center}
  \caption{Recall@1 and F1-Score for different $\varepsilon$ settings of the PGD attack with the different defenses on the CUB200 dataset (Training with the MobileNetV2)}
\label{fig:eps-recall@1-f1-mobi-cub200}
\end{figure}

\textbf{The adversarial robustness of the individual model in the whole ensemble}. As is shown in Figure \ref{fig:recall@1-f1-ind-model-cub200} and Figure \ref{fig:recall@1-f1-ind-model-cars196}, every individual model of the ensemble is still more robust than other defenses and it is better to construct the ensemble and apply our voting mechanism for achieving higher adversarial robustness.

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/f1-ind-model-cub200.png}
% \end{center}
%   \caption{F1-Scores for the individual model of the EAT defense in comparison with other defenses on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:f1-ind-model-cub200}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/recall@1-ind-model-cub200.png}
% \end{center}
%   \caption{Recall@1 for the individual model of the EAT defense in comparison with other defenses on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:recall@1-ind-model-cub200}
% \end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/recall1-f1-ind-model-cub200.png}
\end{center}
  \caption{Recall@1 and F1-Scores for the individual model of the EAT defense in comparison with other defenses on the CUB200 dataset (Training with the MobileNetV2)}
\label{fig:recall@1-f1-ind-model-cub200}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/recall1-f1-ind-model-cars196.png}
\end{center}
  \caption{Recall@1 and F1-Scores for the individual model of the EAT defense in comparison with other defenses on the CARS196 dataset (Training with the MobileNetV2)}
\label{fig:recall@1-f1-ind-model-cars196}
\end{figure}


\subsection{Impact of Hyperparameters}
\textbf{The number of models:} The number of models in the whole ensemble may cause different adversarial robustness. In this work, we study four settings ($N = 1,2,3,4$) on the CUB200 dataset with the MobileNetV2 model. 

As is shown in Figure \ref{fig:recall@1-f1-model-number-cub200}, the adversarial robustness increase with the rising of the number of models. However, there is a little drop in the performance without the attacks and that drop decreases when we increase the number of models.

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/f1-model-number-cub200.png}
% \end{center}
%   \caption{F1-Scores for different model numbers with the EAT method on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:f1-model-number-cub200}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.8\linewidth]{figures/recall@1-model-number-cub200.png}
% \end{center}
%   \caption{Recall@1 for different model numbers with the EAT method on the CUB200 dataset (Training with the MobileNetV2)}
% \label{fig:recall@1-model-number-cub200}
% \end{figure}
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/recall1-f1-model-number-cub200.png}
\end{center}
  \caption{Recall@1 and F1-Scores for different numbers of models with the EAT method on the CUB200 dataset (Training with the MobileNetV2)}
\label{fig:recall@1-f1-model-number-cub200}
\end{figure}

\textbf{The ratio coefficient of the adversarial loss:} The ratio coefficient $\beta$ may cause the influence of the adversarial loss term. In this work, we study five different ratio settings ($\beta = 0, 0.25, 0.5, 0.75, 1$) on CUB200 and CARS196 with the MobileNetV2 model. 

As is shown in Figure \ref{fig:recall@1-f1-beta-cub200} and Figure \ref{fig:recall@1-f1-beta-cars196}, the adversarial robustness is decreasing with the increasing of the $\beta$. At the same time, more powerful robustness causes the drop of the performance without any attacks. That is a trade-off and we select $\beta=0.5$ as the best choice.


\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/recall1-f1-beta-cub200.png}
\end{center}
  \caption{Recall@1 and F1-Score for different $\beta$ settings with the EAT method on the CUB200 dataset (Training with the MobileNetV2)}
\label{fig:recall@1-f1-beta-cub200}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/recall1-f1-beta-cars196.png}
\end{center}
\caption{Recall@1 and F1-Score for different $\beta$ settings with the EAT method on the CARS196 dataset (Training with the MobileNetV2)}
\label{fig:recall@1-f1-beta-cars196}
\end{figure}





